A Longitudinal Multi-modal Dataset for Dementia Monitoring and Diagnosis

Dementia affects cognitive functions of adults, including memory, language, and behaviour. Standard diagnostic biomarkers such as MRI are costly, whilst neuropsychological tests suffer from sensitivity issues in detecting dementia onset. The analysis of speech and language has emerged as a promising and non-intrusive technology to diagnose and monitor dementia. Currently, most work in this direction ignores the multi-modal nature of human communication and interactive aspects of everyday conversational interaction. Moreover, most studies ignore changes in cognitive status over time due to the lack of consistent longitudinal data. Here we introduce a novel fine-grained longitudinal multi-modal corpus collected in a natural setting from healthy controls and people with dementia over two phases, each spanning 28 sessions. The corpus consists of spoken conversations, a subset of which are transcribed, as well as typed and written thoughts and associated extra-linguistic information such as pen strokes and keystrokes. We present the data collection process and describe the corpus in detail. Furthermore, we establish baselines for capturing longitudinal changes in language across different modalities for two cohorts, healthy controls and people with dementia, outlining future research directions enabled by the corpus.

==> cover_letter.tex <==
\section*{Response to the previous reviews.}

We thank the reviewers for their constructive comments.

In our revised version we have made substantial changes and updated the structure of the manuscript emphasizing the introduction of a new multimodal longitudinal corpus consisting of two completed phases each spanning 28 sessions. We further establish baselines for capturing longitudinal changes in language across different modalities in for the two cohorts (controls and people with dementia) mapping possible directions in the field. We believe that these changes have addressed all of the reviewers' comments. Specifically we have made the following revisions:

\begin{itemize}
\item We extend the literature review of existing dementia datasets and the comparative benefits of our new dataset by providing additional aspects, such as the nature of the tasks and ability to elicit linguistic information, the duration of a session etc. (Please refer to Table~\ref{tbl:dataset_review} in Sec.~\ref{sec:introduction}). 
\item We provide additional information about participants' demographics  (Please refer to Sec~\ref{sec:demographics}). This addresses the comments by the 3rd reviewer.  
\item We shorten the analysis and provide substantial statistical information about the collected modalities in the new corpus (refer to Sec.~\ref{sec:datadescription}). This addresses comments by the 2nd reviewer.  
\item We extend the longitudinal analysis by including baselines for the linguistic modalities (i.e., transcribed and typed text data). Please refer to Sec.~\ref{sec:task}. This addresses comments by the 2nd reviewer. 
\item We add a new section to discuss the limitations of the collected corpus. We also discuss future data collection over 3 phases which will be recruiting a new cohort to tackle the relatively small-scaled population in the current collection. This addresses the comments by the 1st reviewer (refer to Sec~\ref{sec:limitations}). We further discuss possible research directions enabled by our corpus. This addresses comments by the 2nd reviewer. We finally discus the particular reasons of dropout between the two collection phases (please refer to Sec~\ref{sec:limitations}). This addresses the comments of the 3rd reviewer.
\item We add another section to discuss the ethics of the study (refer to Sec~\ref{sec:ethical}). This addresses comments by the 3rd reviewer. In this section, we further discuss potential ethical concerns of using spoken language and computational approaches for monitoring and screening changes in cognitive status and dementia. 
\item We have revised the references accordingly. This addresses comments by the 3rd reviewer.
\end{itemize}

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


